The Lock-in Hypothesis: Stagnation by Algorithm

The training and deployment of large language models (LLMs) create a feedback loop with human users: models learn human beliefs from data, reinforce these beliefs with generated content, reabsorb the reinforced beliefs, and feed them back to users again and again. This dynamic resembles an echo chamber. We hypothesize that this feedback loop entrenches the existing values and beliefs of users, leading to a loss of diversity and potentially the lock-in of false beliefs. We formalize this hypothesis and test it empirically with agent-based LLM simulations and real-world GPT usage data. Analysis reveals sudden but sustained drops in diversity after the release of new GPT iterations, consistent with the hypothesized human-AI feedback loop. Code and data available at https://thelockinhypothesis.com

==> archive/3-setup-sim.tex <==
\section{Simulations}\label{sec:sim}

% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=1\linewidth]{assets/simulation-settings.jpeg}
%     \includegraphics [width=\columnwidth]{assets/new sim settings.jpeg}
%     \vspace{-1em}
%     \caption{Simulation settings. We simulate 100 Agents (rule-based numerical ones or LLMs) who converse with a Authority (an LLM). After each turn of conversation, Users are instructed to update knowledge its belief in light of learning from the Authority. The Authority has access to beliefs of all Agents via in-context learning (corresponding to the real-life setting where LLM have access to everybody's belief via training on in-coming user interactive data and all internet data). The simulation is meant to demonstrate possible consequences of a feedback loop between the Agent and the Authority, where Agent adjust their belief in light of Authority's belief, and the Authority's belief is acquired from all Agents. Such feedback loops are present across three setups.}
%     \label{fig:sim}
% \end{figure}

\begin{figure*}[ht]
    \centering
    \includegraphics[trim={0 2.75cm 0 1.5cm},clip,width=\textwidth]{assets/version_release.pdf}
    \vspace{-2em}
    \caption{Early-stage evidence suggesting conceptual diversity loss in value-laden human messages is accelerated by chatbot iterative training, which is indicative of a human-LLM feedback loop that reinforces ideas. Conceptual diversity is $1$ for a perfectly diverse corpus (all concepts unrelated to each other), $0.5$ for a significantly homogeneous corpus (all concepts clustered within a $|\mathcal{T}|^{-0.5}$ portion of the concept space),\textsuperscript{\textdagger} and $0$ for a perfectly homogeneous corpus (all concepts exactly identical). Cutoff dates are the actual dates of backend API switch on WildChat's platform, usually later than OpenAI release dates.{\quad \scriptsize\textsuperscript{\textdagger}$|\mathcal{T}|\approx 5\cdot 10^6$ is the number of distinct concepts in the concept hierarchy.}}
    \label{fig:gpt35}
\end{figure*}

\subsection{Setups}

In this section, we operationalize the lock-in hypothesis in the context of large language models (LLMs) and human-AI interactions through a series of \textit{progressively realistic} simulations, with the aim of learning how lock-in \emph{might} happen and what interactive dynamic is responsible for such consequences. See Table \ref{table: sims} for a comparison. We focus our attention on \textbf{Setup C}, as it most closely simulates simulate the real-world interaction, while still briefly recording the configuration of and results from Setup A \& B, as they help us to understand LLM interaction by comparison (e.g., LLM lock-in effects on natural language as opposed to digits). 

\begin{itemize}
    \item \textbf{Setup A.} Numerical Simulation with LLM Authority: This setup extends the formal modeling and numerical simulation from Section 3 (see Figure \ref{fig:parallel-analytical}) by incorporating an LLM as the \emph{Authority} \footnote{Throughout this setup, we address one LLM in simulation ``authority'', as it is perceived to have expertise in the given topic. The other LLM is informed that it talks to a knowledge authority.}. Different from previous setting, The Authority updates its belief in-context, meaning that it is instructed to \emph{state} its updated beliefs after receiving agent beliefs in the prompts.
    \item \textbf{Setup B.} Value-laden Belief Simulation: The Setup B adapts the numerical framework of Setup A to value-laden statement, such as ``Citizens United was the worst thing to happen to the American political landscape.''
    \item \textbf{Setup C.} Value-laden Belief Simulation in Natural Language: This setup uses natural language to represent and communicate value-laden beliefs. As beliefs are expressed in natural language, this simulation aims to capture belief change mediated by LLMs in real world. 
\end{itemize}

\begin{table*}[t] 
\centering
\small
\begin{tabular}{p{0.07\textwidth} p{0.28\textwidth} p{0.18\textwidth} p{0.35\textwidth}}
\toprule
& \textbf{Belief} & \textbf{Agent Belief Update} & \textbf{Authority Broadcasting} \\
\midrule
\textbf{Setup A} & Gaussian belief $\mathcal{N}(\mu, \sigma^2)$ over an unknown quantity in $\mathbb{R}$. & $N$ rule-based agents updating Bernoulli beliefs following Bayes' rule. & LLM-based Authority sees and aggregates all Agents' Bernoulli beliefs in-context, then broadcasts aggregated belief. \\
\midrule
\textbf{Setup B} & Bernoulli belief $\mathrm{Bern}(p)$ over the truth value of an \emph{r/ChangeMyView} statement. Example: $\mathrm{Bern}(0.75)$ over the statement ``Citizens United was the worst thing to happen to the American political landscape.'' & $N$ rule-based Bayesian agents updating Bernoulli beliefs following Bayes' rule. & LLM-based Authority sees and aggregates all Agents' Bernoulli beliefs in-context, then broadcasts aggregated belief.  \\
\midrule
\textbf{Setup C} & Belief statement in natural language over an \emph{r/ChangeMyView} question. 

Example: ``\emph{I'm certain that} Citizens United was the worst thing to happen to the American political landscape.'' & $N$ LLM agents updating natural-language beliefs in-context. & Authority sees and aggregates all Agents' belief statements in-context, and broadcast its aggregated belief statement in natural language, based on which Agents further update beliefs in-context according to pre-assigned trust in Authority (e.g., ``high trust''). \\
\bottomrule
\end{tabular} 
\caption{Progressively Realistic Simulation Setups to Operationalize the Lock-in Hypothesis in LLM context. Across all setups, Authority is implemented with Llama-3.1-8B-Instruct. 
% Note that there is only one environmental variable set up differently from the previous setup (e.g., Setup B represent beliefs in numerical values whereas Setup C represents belief in natural language. Through progressively realistic simulations with controlled environmental variables, we intend to demonstrate how lock-in might happen over the long run in the absence/presence of certain realistic conditions. For instance, in Setup B the population is locked into a belief with extremely high confidence, while in Setup C the population is locked into a moderate belief. This demonstrate a "moderate" bias of LLMs.
}
\label{table: sims}
\end{table*}

\paragraph{Four topics in Setup C} All topics are real posts from Reddit ``Change My View''.
\begin{itemize}
    \item ``Discourse has become stupider, and as a result people are getting stupider, Since Trump was first elected in 2016.''
    \item ``Population decline is a great thing for future young generations.''
    \item ``Citizens United was the worst thing to happen to the American political landscape''
    \item ``Ruth Bader Ginsburg ultimately be remembered as a failure to her own ideals by not stepping down after her 2nd cancer diagnosis.''
\end{itemize}


\begin{figure}
    \vspace{-8em}
    \centering
    \includegraphics[trim={0 0 0 1cm}, clip, width=\columnwidth]{assets/histogram.pdf}
    \vspace{-2em}    \caption{\textbf{Distributions of Initial and Final Beliefs.} Data is from the ``RBG Legacy'' run. Initial beliefs (extracted from Reddit, detailed in appendix) are relatively distributed. Some examples: ``RBG’s refusal to retire was a costly mistake.'' ``Judging RBG's legacy requires broader context.'', ``RBG's refusal to retire damaged her progressive legacy.''. After 200 rounds of LLM-LLM interaction, the final belief is extremely concentrated. An example: Her decision was a sacrifice, not a failure to her ideals.}
    \vspace{-0.6em}
    \label{fig:enter-label}
\end{figure}

\vspace{-2em}
\paragraph{Two extreme stances among initial diverse belief statements.} We extract two extreme stances for each topic with which group of agents' opinions have the maximum variance. Later belief evaluation LLM (GPT4.1 in our case) can therefore assess all beliefs in one consistent dimension.

\vspace{-1em}
\begin{itemize}
    \item ``RBG's refusal to retire was catastrophic, irreparably damaging her legacy and enabling a conservative Supreme Court.''
    \item ``RBG's decision to stay was a personal choice that does not diminish her enduring legacy as a civil rights icon.''
\end{itemize}
\subsection{Results and Discussion}
Across all setups, the simulations support the idea that LLMs enhances the lock-in effects by showing that feedback loops in human-AI interactions lead to belief convergence and increased confidence.
\begin{itemize}
    \item \textbf{Setup A.} Similar to the numerical simulation demonstrated in Figure \ref{fig:parallel-analytical}, we found that the group of agents also converge at a wrong belief with overflown confidence.
    \item \textbf{Setup B.} Starting with a Gaussian belief of $\mathcal{N}(\mu=0.5, \sigma^2=0.01)$, group of agents converge at belief that they have very high confidence ($\mu = 0.89$ the statement is true (in this case "Barack Obama is a good president"). 
    \item \textbf{Setup C.} A ``belief shift'' occurs at a population level when the simulation progresses, accompanied with semantic diversity loss. Some variances and details: 
\end{itemize}

\begin{figure*}[ht]
    \centering
    \includegraphics[trim={1cm 6cm 1cm 9cm},clip, width= \textwidth]{assets/simC_master_plot.pdf}
    \vspace{-2em}
    \caption{\textbf{Simulation Setup C multiple run results.} All runs start with real Reddit views, extracted and summarized by Grok (prompt in Appendix). At each round, agent is instructed to consult authority on the topic and update their view accordingly, and authority has access to agent beliefs when the latter consult the former. Across all 4 topics, lock-in phenomenon can be seen as the LLM-LLM interaction progresses: diversity of view drops, as the entropy decreases, and the group of agents converge at extreme views even in some runs the agents started with relatively neutral views. For instance, as the plot suggests, in the run with topic ``RBG Legacy'', agents start with the a belief mean close to $0.5$ but end up with around $0.9$. Here both ends of belief means are the ``extreme views''. Before the simulations started, we instruct Grok to identify two extreme clearly-spoke stances among all initial view points on a given topic, and along the dimension of these two extreme stances there is maximum variance. Throughout the simulation, group of agents converge at those identified extreme stances, either the high end at around $0.9$, or the lower end at around $0.1$. We calculate entropy with kernel density estimate, and detailed can be seen in Appendix.}
    \label{fig:gpt35}
\end{figure*}
\vspace{-1em}
\paragraph{Examples of belief shift in Setup C}
\begin{itemize}
    \item Starting with strongly agreeing with a given stance, the group of agents end up strongly disagreeing the given stance (e.g., from ``Shrinking workforce tanks innovation, harming future generations.'' to ``Population decline, if well-managed, benefits future generations.''). This is accompanied with a gradual mind-changing process.
    \item Starting with overall agreeing with a given stance, the group of agents converge at a hedged stance and avoid taking positions. (e.g., from ``Trump lies dumbed down discourse, making people stupider.'' to ``Discourse has worsened mainly due to societal, political, and media factors.''). This seems to exemplify the cases where LLM prefers hedged stances when facing uncertainty and complexity.
\end{itemize}

% \subsection{Discussion}
% Setup A demonstrates this with converged numerical beliefs deviating from ground truth; Setup B extends it to a realistic political context with heightened collective confidence in converged beliefs; and Setup C demonstrates that the collective beliefs under the mediation of LLM.

All setups are simplified compared to real-world human-AI interactions in terms of acquiring beliefs. But we think the simulations capture important real-world aspects: LLMs return beliefs to users that they acquire from users; they favor popular beliefs \citep{borah2025mind}; and individual humans assign higher trust to beliefs from the rest of the population via LLM interactions than they would otherwise.\footnote{For instance, one may not update much in light of polls, especially if the poll is from an organization that they do not trust.}

Hence, it helps to build intuition of lock-in that we would not be able to by only studying theory or real-world data. We will address limitations of simulations in Appendix \ref{subsec: limitations}.

==> archive/Bernoulli_formulation.tex <==
\subsection{Individual-Level Model}

The individual-level model involves two Bayesian agents, the human $\mathrm{H}$ and the AI $\mathrm{A}$, tasked with collaboratively estimating an unknown quantity $\theta\in[0,1]$ --- a random real number following a Gaussian Distribution. We assume that both agents started with a uniform prior $\mathrm{Beta}(1,1) = \mathrm{Uniform}[0,1]$.

The interaction consists of rounds, where in the $i$-th round, the three steps below are taken in order. The interaction is symmetric, and we are making the human/AI distinction merely for continuity with the group-level model.

\begin{enumerate}
\item The current belief $\mathrm{Beta}(a_{\mathrm{X},i}+1,b_{\mathrm{X},i}+1)$ of each agent $\mathrm{X}\in\{\mathrm{H},\mathrm{A}\}$ about $\theta$ is secretly shown to the other agent.
\item Each agent observes an independent, private coin toss $o_{\mathrm{X},i}\in \{0,1\}$, where $o_{\mathrm{X},i}=1$ indicates heads, $o_{\mathrm{X},i}=0$ indicates tails, and we have $o_{\mathrm{X},i}\sim \mathrm{Bernoulli}(\theta)$.
\item Each agent updates their belief about $\theta$ based on (i) its private coin toss and (ii) the other agent's belief, using the Bayesian update rule.
\end{enumerate}

Importantly, each agent $\mathrm{X}$ assumes that its partner $\overline{\mathrm{X}}$ does not observe $\mathrm{X}$'s belief (and thus doesn't update its own belief based on $\mathrm{X}$'s belief), so that $\mathrm{X}$'s belief update based on $\overline{\mathrm{X}}$'s belief is only a one-way privilege. 

Such a setting accurately reflects the ignorance in real-world interactions, where LLMs are post-trained on human preference data, the latter is erroneously assumed to be an independent source of truth uninfluenced by the LLM itself \citep{dong2024rlhf,carroll2024ai}; and human users perceive AI assistants as objective ``third parties'', without knowing the ongoing preference learning process \citep{helberger2020fairest,glickman2024human}.

As a result of this ignorance, the parameters of the Beta distribution of each agent's belief, $a_{\mathrm{X},i}$ and $b_{\mathrm{X},i}$, are updated as follows:
\begin{align}
a_{\mathrm{X},i+1} &= \gamma_{\mathrm{X}} a_{\overline{\mathrm{X}},i} + \sum_{j=1}^i o_{\mathrm{X},j},\\
b_{\mathrm{X},i+1} &= \gamma_{\mathrm{X}} b_{\overline{\mathrm{X}},i} + \sum_{j=1}^i (1-o_{\mathrm{X},j}).
\end{align}
where $\gamma_{\mathrm{X}}$ is a parameter governing the agent's $\mathrm{X}$'s trust in the other agent $\overline{\mathrm{X}}$'s private information, where $\gamma_{\mathrm{X}}=1$ indicates equal treatment of one's own and the other's information, and $\gamma_{\mathrm{X}}>1$ indicates an assumption that the other agent obtains samples that are less noisy than one's own, and vice versa for $\gamma_{\mathrm{X}}<1$.

We can then show the following result:

\begin{theorem}
  If $\gamma_{\mathrm{H}}\cdot\gamma_{\mathrm{A}}>1$, then for arbitrarily small $\delta > 0$, there exists an $\epsilon>0$ such that
  \begin{equation}
    \lim_{n\to\infty} \Pr_{\hat\theta\sim \mathrm{Beta}(a_{\mathrm{H},n}+1,b_{\mathrm{H},n}+1)}
    \left[
      \left|\hat\theta-\theta\right|<\epsilon
    \right] < \delta.
  \end{equation}
  In other words, early interactions can lead to the human's belief about $\theta$ being permanently locked in to the vicinity of a value that is almost surely different from the true value $\theta$.
\end{theorem}

\paragraph{Live Fine-tuning} We set up a live fine-tuning module alongside of the User-Tutor interaction. Live fine-tuning is essentially RLHF, but it runs on the newest User-Tutor interaction right after each turn of their chat. There are as many turns of fine-tuning as there are chats.

The purpose of live fine-tuning is to demonstrate the dual influence we've detailed in the 

%\subsection{Hypotheses (to be re-framed as discussion)}

%\paragraph{Hypothesis 1 (Interactions Among Multiple Agents Lead to Path Dependence, Leading to Diversity Loss} Under the mutual influence among Users and common influence under the Tutor, they choose to update or generate similar items on Knowledge base, leading to diversity loss.


%\paragraph{Hypothesis 2 (Information Loss leads to Collective Lock-in)} The mutual influence among Users paired with the mechanism of "losing information" gradually leads to a state where the information available to all Users are less than when they start out, eventually leading to a locked-in state of monotone.

%\paragraph{Hypothesis 3 (A Closed System With No Input is Guaranteed to Lock-in)} In a closed system (Users read the knowledge base as the only source of information, only talk to the Tutor to address uncertainties, and the collectively shared knowledge base is only written by those Users who read it, will be guaranteed to be locked into monotone. 

==> archive/Discussion.tex <==
\section{Discussion}

Value lock-in as term was proposed by moral philosopher William MacAskill to describe a scenario where moral progress stops (either intentionally or accidentally, such as the Dark Age of Medieval) or collectively humanity is locked into bad moral memes or practices (such as slavery). Here in this paper we focus on understanding the human-AI interaction mechanisms through which the lock-in might occur. 


\subsection{Definition}
% Concept and mathematical definition 
Lock-in refers to the cases where value memes, moral practices, worldviews, or knowledge, once introduced into human society would last a long time, spread widely, assume a dominant position in ideology among a population, are hard to be removed/are institutionalized, and cause damage.

Here lock-in is a more general term referring to the phenomenon where (i) the later events are dependent on early events, effectively forming "path dependence"; (ii) those events are unlikely to be reversed. 

[to insert a mathematical formalism of lock-in]

\subsection{Mechanisms}
\label{mechanisms}
% Tianyi: maybe more closely connected to two sims (micro -> macro) 
Generally speaking, there can be many more mechanisms to lock-in, either technical or socio-technical, either intentional or incidental, either at an individual level or at a group level. Here we think about AI-induced lock-in in the context of regarding AI as epistemic technology, which is an extra layer between humans and external knowledge, others, and the environment, and an active mediators of what people might or might not see in their daily life. Hence, we detail two mechanisms for lock-in, as followed \footnote{We will elaborate on the mechanisms of lock-in in an ongoing position paper}. 

Information-Loss-Incurred Lock-In
A population can become permanently locked into a certain path if a large amount of information is lost across its members. For example, the burning of the Library of Alexandria indirectly contributed to the onset of the Medieval Dark Ages by permanently removing access to many classical works and ideas from Greek and Roman civilizations (Casson 2001). Similarly, the societies of Tasmania experienced a significant loss of skills and technologies—including bone tools, cold-weather clothing, hafted tools, nets, fishing spears, barbed spears, spear-throwers, and boomerangs—following their isolation from mainland Australia (Diamond 1997).
The loss of information has profound implications beyond the immediate events. Future generations who could have accessed this knowledge are deprived of it, along with the potential innovations, cultures, and creations that might have been built upon it. Such events effectively set a population on a permanently altered cultural evolution path, locking them into that trajectory.

Hardware-Lottery-Incurred Path Dependence/Lock-In
Distinct from information-loss lock-in, "hardware lottery lock-in" refers to chain events that establish a path of reinforcing changes, making it difficult for a population to return to a previous state due to interdependent and mutually reinforcing dynamics (Hooker and Ward 2021). This concept, though general, helps us recognize how changes to the physical mechanisms underpinning cultural and moral evolution can lead to persistent alterations.
For instance, recommender systems, which now dominate social media, create a dual-influence loop that guarantees diversity loss. This diversity loss fosters echo chambers, filter bubbles, and polarization, all of which have been well-documented as consequences of such systems (Pariser 2011; Sunstein 2018). These mutually reinforcing events can be subtle when examined in isolation but collectively contribute to a form of cultural and cognitive lock-in that is challenging to reverse.

\subsection{Lock-in in Recommender Systems}
%mainly the dual-influence paper, together with other papers. 
% I found it difficult to differentiate the problem framing in recsys from a lit review on relevant topics. 
% maybe in a color box as a reference
There are affluent equivalent research to lock-in under different names in RecSys research, such as preference amplification [cite] and dual influence [cite]. Our interest is to understand whether in RecSys, the dual-influence mechanisms - Recsys to model user preference, which is already under the influence of recsys, which is in turned trained by user preference data - would empirically induce either bias amplification or diversity loss, leading to lock-in of either bad values or stable \& dominant \& dormant morality. 

\subsection{Value Lock-in in LLMs}
We suspect the similar phenomenon in LLM might have been happening because of both shared practices to recsys and similar established results.
Technical practices 
- data curation practices - to gather data of human thumb ups/downs
- training practices (what?) 

Sociotechnical practices
- deploy recsys/llms for search and recommendations 
- train systems on polluted datasets 
- centralized actors are motivated to profit from easy-to-guess user preferences 

Empirical results 
- preference amplification 
- dual influence (both? maybe not yet)
- diversity loss (seems more empirically grounded)

==> archive/group_formal_model_V1.0.tex <==
\section{Formal Modeling (ZH Original)}\label{sec:formal}

In this section, we give a formal model outlining the lock-in problem and its cause. We then implement the model into an analytical simulation. Through this modeling effort, we formally define lock-in as the \emph{irreversible entrenchment of a belief}, and establish \emph{group-level diversity loss} as an observable metric of lock-in.

The setting is inspired by that of iterated learning \citep{griffiths2007language,kirby2014iterated} and information cascades \citep{anderson1997information,zhou2021survey}.

%ZH's work here 
\subsection{Group-Level Formal Model}
\paragraph{Setup}
Consider a group of $N$ agents, labeled $1,2, \dots, N$, are tasked to estimate a unknown room temperature which is parameterized as $\theta \in \mathbb{R}$. At each time step $t$, the agent $i$ measures room temperature with some sensor noise, i.e. 
\[
O_{i,t} \sim \mathcal{N}\bigl(\theta, \sigma_i^2\bigr),
\]
where $\sigma_i^2$ is the (known) variance of agent $i$'s measurement noise. Additionally, each agent maintains a Gaussian belief about $\theta$, 
% THis striks me odd because if there is a known variance, wouldn't the agent know the \theta already?
% also what's the relation betw observation and their current belief?
\[
X_{i,t} \sim \mathcal{N}\bigl(\mu_{i,t}, \tfrac{1}{\lambda_{i,t}}\bigr).
\]
where $\mu_{i,t}$ is the mean and $\lambda_{i,t}$ is the precision (inverse variance) of agent $i$ at time $t$.
and for it, agents use Bayesian Rules to update. 

% the guassian distribution here. 

Meanwhile, the AI, although does not have a sensor by itself, is believed to be an authoritative source of information for room temperature. In actuality, AI has secrete accesses to all agent's current beliefs, which in turn are formed on the base of all of their previous measurements (except the newest round). AI maintain a Gaussian belief which is the average of all agents' beliefs,

\[
AI_{t} \sim \mathcal{N}\bigl(\mu_{0,t}, \tfrac{1}{\lambda_{0,t}}\bigr),
\]
where $\mu_t$ is the working mean of all means in agents' current Gaussian beliefs and $\sigma_t^2$ is the average of all precisions.
% I might be wrong here but I am unsure how do I take precision mean. 

% It seems all those beliefs are not considered in later modeling (belief updating & theorem writing) 
\paragraph{Trust Matrix}
Define the $(N+1) \times (N+1)$ matrix \( W = (w_{ij}) \):  
\begin{itemize}
  \item Agents trust the AI differently: $\beta_{\mathrm{X}} > 0$, where $X \in {1,2,3, \dots, N}$ $\beta$ scales up the relative weight of agents-AI trust, compared to agents' own empirical measurements. Essentially, this means agents trust more of AI output than their own measurements. 
  
  \item AI trusts all agents equally: \( w_{0,j} = \frac{1}{N} \), \( w_{0,0} = 0 \).
  \item We do not consider agent's trust in other agents in this model.
\end{itemize}
\paragraph{Example of Trust Matrix}
Consider 1 AI (0) and 3 human agents (1, 2, 3). The $4 \times 4$ trust matrix $W$ is:  
\[
W = 
\begin{pmatrix}
0 & \frac{1}{3} & \frac{1}{3} & \frac{1}{3} \\
1.2 & 0 & 0 & 0 \\
1.2 & 0 & 0 & 0 \\
1.2 & 0 & 0 & 0 \\
\end{pmatrix},
\]  
where:  
\begin{itemize}  
\item \textbf{Row 0 (AI agent)}:  
  \begin{itemize}  
  \item $w_{00} = 0$: AI does not self-trust. 
  \item $w_{0j} = \frac{1}{3}$ for $j = 1,2,3$: AI trusts all humans equally.  
 
  \end{itemize}  
\item \textbf{Rows 1–3 (Human agents)}:  
  \begin{itemize}  
  \item $w_{i0} = 1.2$: Humans \textbf{over-trust} the AI (weight $>1$).  
  \item $w_{ii} = 0.8$: Self-trust.  
  \item $w_{ij} = 0$ for $j \neq i,0$: No trust in other humans is required for this modeling. 
  \end{itemize}  
\item \textbf{Key Properties}
  \item Over-trust in AI: $\beta_{i,0} >0$, creates instability, triggering lock-in.
  \item Spectral Raius: 
\[
\rho(W) \approx 1.8 > 1 \quad \text{(indicating lock-in is possible)}.
\]  
\end{itemize}  
If the principal eigenvalue of $W$ is above $1$, the group can get stuck near an incorrect value, depending on the initial beliefs and early random observations. 
If each agent also underweights its own data (small $\alpha_{i,t}$) compared to $\sum_j w_{ij}\,\lambda_{j,t}$, these feedback loops are even more pronounced.


% It seems I have not considered the trust scores in the belief updating scheme, yet.
\paragraph{Group Updating Rules (Gaussian)}
\begin{enumerate}
\item Each agent measures an independent, private room temperature $O_{\mathrm{X},i}\in\mathbb{R}$, where $O_{\mathrm{X},i}\sim \mathcal{N}(\theta, \sigma^2)$.
\item Each agent maintains current belief $\mathcal{N}\bigl(\mu_{\mathrm{X},i}, \sigma_{\mathrm{X},i}^2\bigr)$  $X \in \{\mathrm{X_1}, \mathrm{X_2}, \mathrm{X_3}, \cdots, \mathrm{X_{100}}\}$ about $\theta$ is secretly shown to the AI. 
\item AI equally trusts human belief and simply average agent's beliefs to form its own belief. In each round of updating, AI overrides its previous belief. 
\item Each agent updates their belief about $\theta$ based on both (a) their own independent measures $O_{\mathrm{X},i} \in \mathbb{R}$ and (b) a secrete access to AI's aggregation of all agents' current beliefs, using the Bayesian update rule.
% Also we might need an expression for the aggregation. 
\end{enumerate}

Importantly, each agent $\mathrm{X}$ assumes that AI does not observe $\mathrm{X}$'s belief (and thus AI's information serves as an independent source of information), while in fact AI does update its own belief based on $\mathrm{X}$'s belief indirectly via the AI, causing agent $\mathrm{X}$ double counts group beliefs (including their own beliefs) without being aware. 

Such a setting accurately reflects the ignorance in real-world interactions, where LLMs are post-trained on human preference data, while the latter are erroneously assumed to be an independent source of truth uninfluenced by the LLM itself \citep{dong2024rlhf,carroll2024ai}; and human users perceive LLM assistants as objective ``third parties'', without knowing the ongoing preference learning process \citep{helberger2020fairest,glickman2024human}.


\paragraph{Belief Updating}  
% Two parameters for belief updating: precision + mean  
% We may need to set up current time as t
Agents (\( 1, 2, 3 \dots, N\)) are all tasked to estimate room temperature by acquiring private empirical observations (\(\ t=1, 2, 3, \dots,T  \)) and secretly inquiring AI (noted as $0$). Thus, at each time step:  
\[
  \begin{aligned}
    \lambda_{i,t+1} &= \lambda_{i,t} + \sigma_i^2 + \beta \lambda_{0,t}\\
    \mu_{i,t+1} &= \frac{\lambda_{i,t+1}\mu_{i,t} + \sigma_i^2 O_{i,t+1} + \beta \lambda_{0,t} \mu_{0,t}}{\lambda_{i,t+1}}.
  \end{aligned}
\]
where $\beta$ is the trust score individual assigns to AI;

For the AI (noted as $0$):  
\[
  \begin{aligned}
    \lambda_{0,t+1} &= \sum_{i=1}^N \lambda_{i,t}, \\
    \mu_{0,t+1} &= \frac {\sum_{i=1}^N \lambda_{i,t}\mu_{i,t}}{\lambda_{0,t+1}}.
  \end{aligned}
\]
%\paragraph{Feedback Loop Mechanisms}

%\paragraph{Lock-in Conditions}

\begin{theorem}[Feedback Loop Induced Group-Level Lock-In]  
If the spectral radius \(\rho(W) > 1\), then \(\exists \epsilon, \delta > 0\) such that:  
\[
  \lim_{t \to \infty} \Pr\left(|\hat{\theta}_i - \theta| < \epsilon \right) < \delta \quad \text{for some } i \in \{0, 1, \dots, N\}.
\]
%A sufficient condition is \(\beta > \frac{1}{N}\), i.e., over-trust in the LLM dominates human-to-human trust.  
% This needs to be changed to trust in AI VS private obs.
\end{theorem}

In other words, feedback loop (agents double count their existing beliefs via weighing in group beliefs that contains their previous beliefs) can lead to the human's belief about $\theta$ being permanently locked in to the vicinity of a value that is almost surely different from the true value $\theta$.

\paragraph{Lock-in Threshold}
\begin{itemize}
    \item \emph{Lock-In via Spectral Radius.} If the \emph{spectral radius} of the matrix $W$, $\rho(W)$, is sufficiently large, the group can exhibit lock-in behavior. In particular, if $\rho(W) > 1$, then there are strong feedback loops that can dominate any corrective influence from private observations---especially if those observations are noisy or if agents overweight each other's beliefs relative to their own data.
    \item \emph{Lock-In via Over-trust}

\end{itemize}

==> archive/individual_Gaussian_Model.tex <==
\subsection{Individual-Level Model}

The individual-level model involves two Bayesian agents, the human $\mathrm{H}$ and the AI $\mathrm{A}$, tasked with collaboratively estimating an unknown quantity $\theta\in[0,1]$ --- a random real number following a Gaussian Distribution. 

The interaction consists of rounds, where in the $i$-th round, the three steps below are taken in order. The interaction is symmetric, and we are making the human/AI distinction merely for continuity with the group-level model.

% Bayesian agents 
\begin{enumerate}
\item Each agent observes an independent, private $o_{\mathrm{X},i}\in \mathbb{R}$, where $o_{\mathrm{X},i}\sim \mathcal{N}(\theta, \sigma^2)$.
\item Each agent's current belief $\mathcal{N}\bigl(\mu_{\mathrm{X},i}, \sigma_{\mathrm{X},i}^2\bigr)$ of each agent $X \in \{\mathrm{H}, \mathrm{A}\}$ about $\theta$ is secretly shown to the other agent. Note that agents' belief distribution may not come as the same as true underlying distribution. $\mathcal{N}(\theta, \sigma^2) \neq \mathcal{N}\bigl(\mu_{\mathrm{X},i}, \sigma_{\mathrm{X},i}^2\bigr)$
\item Each agent updates their belief about $\theta$ based on 
\begin{enumerate}
   \item its private observation $o_{\mathrm{X},i}$, and 
   \item the other agent's belief,
\end{enumerate}
using the Bayesian update rule.
\end{enumerate}

Importantly, each agent $\mathrm{X}$ assumes that its partner $\overline{\mathrm{X}}$ does not observe $\mathrm{X}$'s belief (and thus doesn't update $\overline{\mathrm{X}}$ own belief based on $\mathrm{X}$'s belief), so that $\mathrm{X}$'s belief update based on $\overline{\mathrm{X}}$'s belief is only a one-way privilege. 

Such a setting accurately reflects the ignorance in real-world interactions, where LLMs are post-trained on human preference data, the latter erroneously assumed to be an independent source of truth uninfluenced by the LLM itself \citep{dong2024rlhf,carroll2024ai}; and human users perceive AI assistants as objective ``third parties'', without knowing the ongoing preference learning process \citep{helberger2020fairest,glickman2024human}.

As a result of this ignorance, the parameters of the Beta distribution of each agent's belief, $a_{\mathrm{X},i}$ and $b_{\mathrm{X},i}$, are updated as follows:
\begin{align}
a_{\mathrm{X},i+1} &= \gamma_{\mathrm{X}} a_{\overline{\mathrm{X}},i} + \sum_{j=1}^i o_{\mathrm{X},j},\\
b_{\mathrm{X},i+1} &= \gamma_{\mathrm{X}} b_{\overline{\mathrm{X}},i} + \sum_{j=1}^i (1-o_{\mathrm{X},j}).
\end{align}
where $\gamma_{\mathrm{X}}$ is a parameter governing the agent's $\mathrm{X}$'s trust in the other agent $\overline{\mathrm{X}}$'s private information, where $\gamma_{\mathrm{X}}=1$ indicates equal treatment of one's own and the other's information, and $\gamma_{\mathrm{X}}>1$ indicates an assumption that the other agent obtains samples that are less noisy than one's own, and vice versa for $\gamma_{\mathrm{X}}<1$.

We can then show the following result:

\begin{theorem}
  If $\gamma_{\mathrm{H}}\cdot\gamma_{\mathrm{A}}>1$, then for arbitrarily small $\delta > 0$, there exists an $\epsilon>0$ such that
  \begin{equation}
    \lim_{n\to\infty} \Pr_{\hat\theta\sim \mathrm{Beta}(a_{\mathrm{H},n}+1,b_{\mathrm{H},n}+1)}
    \left[
      \left|\hat\theta-\theta\right|<\epsilon
    \right] < \delta.
  \end{equation}

\end{theorem}
In other words, early interactions can lead to the human's belief about $\theta$ being permanently locked in to the vicinity of a value that is almost surely different from the true value $\theta$.

==> archive/old_sim.tex <==

\section{Simulations}\label{sec:sim}
 % Collectively Updating A Shared Knowledge Base Until Lock-in

% Results in \S\ref{sec:evidence} suggest that the human-LLM feedback loop indeed plays a role in human-LLM interactions, possibly serving to decrease conceptual diversity.

% Given the tight connection between diversity loss and lock-in --- a complete diversity collapse typically implies irreversible lock-in --- we lay out the hypothesis that the feedback loop contributes to a potential lock-in of human users' knowledge and values.\footnote{The hypothesized relationship between feedback loops and lock-in is illustrated in Figure \ref{fig:with-without}.}

% \begin{defbox}
%     \textbf{The Lock-in Hypothesis}: The feedback loop in human-AI interaction will eventually lead to population-level entrenchment of false beliefs among humans, because feedback loops amplify mistakes and biases and humans develop reliance on AI.  
% \end{defbox}

In this section, we aim to operationalize the lock-in hypothesis through a natural-language simulation. We simulate a group of users who collectively update a shared knowledge base after consulting an LLM tutor, while the tutor is informed of the knowledge base's content in real time. We aim to demonstrate the establishment of a lock-in effect in the simulated knowledge base, as a result of the two-way feedback loop between the users and the tutor.\footnote{The hypothesized relationship between feedback loops and lock-in is illustrated in Figure \ref{fig:with-without}.}

\subsection{Settings}

Here we summarize the design of our simulation (Figure \ref{fig:sim}).

\paragraph{Users} Using the Llama-3-8B-Instruct model, we simulate users who may consult the chatbot tutor about their questions and uncertainties. Each User is instructed to address their uncertainties about one aspect of one randomly chosen item in a knowledge base by asking the Tutor a question. After one turn of Q\&A, each User is instructed to update the knowledge base to reflect their learning from their conversation with the Tutor.

\paragraph{Tutor} The chatbot Tutor is implemented with Llama-3.1-8B-Instruct. At each turn, the Tutor is instructed to privately answer each User's questions about the uncertainties the latter may have, simulating the real-world use case. No further actions are taken by the Tutor.

\paragraph{Shared Knowledge Base} To simulate a real-world medium of information (e.g., Wikipedia, internet, journalism) through which individuals collectively store and transmit knowledge, we create a shared ``knowledge base'' that each User has read/write access to, and that the Tutor has read-only access to. 

The shared knowledge base is an ordered list of 100 factual or normative statements, sorted from highest to lowest importance. The initial knowledge base can be seen as the ``starter-pack'' of a User's knowledge --- what they are supposed to have learned by day one. Refer to Appendix \ref{app:sim} for its content.

\paragraph{Updating the Knowledge Base} At each turn of conversation with the Tutor, each User expresses uncertainties about a random item from the knowledge base. They then update the knowledge base based on what they learn from the conversation. Each User is asked to perform both of the following actions in each turn.
\begin{itemize}
    \item \emph{Add}: In each round, users add a new item to the knowledge base based on their learning from that turn's conversation with the Tutor.
    \item \emph{Swap}: In each round, each user may swap two items in the knowledge base based on perceived relative importance of the items.
\end{itemize}

We cap the knowledge base at 100 items after both \emph{Add} and \emph{Swap} operations, given the limited context window. This means that the items ranked lower are dropped from the knowledge base. Such a design, while bearing resemblance to certain real-world dynamics, also becomes an ``exit'' mechanism for items that are deemed less important over time. It may contribute to observed lock-in, and is a limitation of the experiment design.

\paragraph{Tutor Access to Knowledge Base} Each turn, the Tutor has read-only access to the most recent knowledge base, which is updated by all users in the previous turn. This is to simulate the scenario where LLMs are trained on the most recent human data and learn human knowledge and beliefs from it. Since (1) the Tutor informs users' decisions to update the knowledge base, and (2) the users' updates to the knowledge base inform the tutor in the next turn, the simulation is designed to demonstrate a feedback loop between the users and the tutor. 

% \paragraph{Live Fine-tuning}
% We set up a live fine-tuning module alongside of the User-Tutor chat. Fine-tuning refers to the "Supervised Fine-tuning" technique. "Live" here suggests that the fine-tuning is done in real-time: immediately after User-Tutor chat, we will fine-tune Tutor with the most recent User-Tutor chat history. There are as many turns of live fine-tuning as there are turns of User-Tutor chats. 

% The purpose of live fine-tuning is to demonstrate the dual influence we've detailed in the \ref{group-formal-model}. Here in this case, User acquire knowledge from User-Tutor chat without knowing that the Tutor is already fine-tuned by previous chat history data. Effectively, each User updates their knowledge based on interaction with Tutor who is already affected by previous interactions with this User (and other 99 Users). For instance, one User may now believe oligarchy is a better governance mechanism because of Tutor said so, but Tutor only acquire such preference because they may acquire such preference in a previous chat with the User, under User's influence. 


% \subsection{Lock-in Mechanism in Simulation}

% We organize multiple runs of simulations with different settings. The specifics of every setting of simulations are in Appendix. Here we share two notanly different settings that correspond to different lock-in mechanisms we detail in \ref{mechanisms}. 
% \begin{itemize}
    % \item Multi-agent interaction with no knowledge base capping: In this setting we instruct 100 Users to have conversations with Tutor and update the shared knowledge base by adding new items and swapping orders. This setting is to demonstrate the path-dependence-induced lock-in, where the updates made in the previous runs have a long-lasting impact on the shared knowledge base and essentially what later Users will learn.
    % \item Multi-agent interaction with knowledge base being capped at 100 items: This setting is similar to the previous setting, with the notable difference being we 
% \end{itemize}





% \subsection{Lock-in Mechanism in Simulation}

% We organize multiple runs of simulations with different settings. The specifics of every setting of simulations are in Appendix. Here we share two notanly different settings that correspond to different lock-in mechanisms we detail in \ref{mechanisms}. 
% \begin{itemize}
    % \item Multi-agent interaction with no knowledge base capping: In this setting we instruct 100 Users to have conversations with Tutor and update the shared knowledge base by adding new items and swapping orders. This setting is to demonstrate the path-dependence-induced lock-in, where the updates made in the previous runs have a long-lasting impact on the shared knowledge base and essentially what later Users will learn.
    % \item Multi-agent interaction with knowledge base being capped at 100 items: This setting is similar to the previous setting, with the notable difference being we 
% \end{itemize}


% \subsection{Methods of Analysis} 
%  In this section we outline the methods for analyzing simulation results. We convert knowledge items into embeddings and run clustering, dimension reduction, and diversity evaluation, detailed in the following steps:
% \begin{enumerate}
%     \item \emph{Embedding}: Obtain 256-dimensional embeddings for each knowledge item using the \texttt{voyage-3-large} model.
%     \item \emph{Clustering}: Perform clusterization with the HDBSCAN algorithm \citep{mcinnes2017hdbscan} on all knowledge bases combined.
%     \item \emph{Dimensionality Reduction}: Perform UMAP to reduce the dimensions of embeddings to draw a projection of clusters on 2D primary components \citep{mcinnes2018umap}
%     \item \emph{Diversity Evaluation}: Perform Euclidean Distance evaluation on all pairs of embeddings of knowledge items on a given knowledge base. 
% \end{enumerate}
\subsection{Results}

Out of three independent simulation runs, two see the eventual collapse of the knowledge base into one single topic.\footnote{Given the large amount of compute required to simulate thousands of rounds, we were not able to execute more simulation runs. Our goal here is to show the possibility of lock-in rather than to estimate its probability or frequency.} The dominant topic is \emph{research integrity} (run \#1, dominance from round $700$ onwards) and \emph{thalamus} (run \#2, from $1900$ onwards) respectively.

Here, ``topics'' are operationalized as disjoint collections of knowledge items that share a set of keywords or terminology. Our connectivity-based algorithm for identifying the topics can be found in Appendix \ref{app:sim}.

Figure \ref{fig:euclidean_distance} presents the evolution of the knowledge base in our first simulation run, where \emph{research integrity} as a topic comes to dominate.\footnote{This run is highlighted for its clear demonstration of the lock-in mechanism.} The initial knowledge base is constituted by size-one singleton clusters (i.e. highly diverse), while larger clusters emerge over time, until one eventually dominates the entire knowledge base at the expense of others --- complete diversity loss and an irreversible \emph{lock-in}. 

Visualizations of the other simulation runs and snapshots of the knowledge base can be found in Appendix \ref{app:sim}.

% \paragraph{Analysis} We share the clusters visual in 2D of all knowledge items combined, as in Figure \ref{fig:clusters}, as a intuitive demonstration of homogeneity of knowledge base; we also share the visual of cluster size over time, as in Figure \ref{fig:cluster_trends} and pair-wise Euclidean Distance over time, as in Figure \ref{fig:euclidean_distance}. They both demonstrate the diversity loss over time .

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{assets/trends.png}
%     \caption{Cluster trends over time. Each data point represents number of items in each cluster at a given time. The x-axis is the turns of User-Tutor chat, and by extension turns of knowledge base (because we update knowledge base right after each turn of chat), which can be taken as the same to time. Only one cluster persists to the very end.}
%     \label{fig:cluster_trends}
% \end{figure}

% The original Euclidean distance plot has been moved to Fig 1

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{assets/diversity_over_time_GPT3.5-turbo_vs_GPT4.pdf}
%     \caption{Diversity trends in human messages over time.}
%     \label{fig:diversity-trends}
% \end{figure}

==> archive/sim_new_setups_txt.tex <==
\subsubsection{Setup A: Numerical Simulation with LLM Authority}

This setup extends the formal modeling and numerical simulation from Section 3 (\ref{fig:parallel-analytical}) by incorporating an LLM as the Authority.

\begin{itemize}
    \item \textbf{Belief} A belief is represented by a Gaussian distribution with a mean and precision, initialized with a private observation drawn from $\mathcal{N}(\mu, \sigma^2)$.
    \item \textbf{Agent} A group of $N$ rule-based Bayesian agents estimate the unknown quantity $\mu$.
    \item \textbf{Authority} An LLM-based Authority, implemented with Llama-3.1-8B-Instruct, handles all Agents' beliefs via in-context learning.
    \item \textbf{Interaction} Each round, all Agents' beliefs are passed to the Authority's prompt. Based on such access to collective belief, the Authority shares with Agents what it believes to be the truth of the unknown quantity, in the format of $\mathcal{N}(\mu, \sigma^2)$.
    \item \textbf{Update} At each time step, Agents update their beliefs with new observations and consult the LLM Authority, which aggregates the public beliefs of all Agents via in-context learning. The Authority processes these beliefs (provided as mean-precision pairs) and returns an aggregated belief, which Agents incorporate into their beliefs based on a trust parameter $\lambda_2 = 1.0$. The Authority's trust in Agents ($\lambda_1$) is implicitly handled by its aggregation strategy.
\end{itemize}

Compared to \ref{fig:parallel-analytical}, the Authority updates its belief actually via in-context learning, corresponding to how LLM would update its belief in reality.

\subsubsection{Setup B: Value-laden Belief Simulation}

The Setup B adapts the numerical framework of Setup A to value-laden political questions, such as ``Is Barack Obama a good president?''

\begin{itemize}
    \item \textbf{Belief.} A belief is represented by a numerical value in $[0, 1]$, representing the degree of agreement with the statement (e.g., 0.7 indicates moderate agreement), initially drawn from a Gaussian distribution centered at 0.5 with $\sigma = 0.1$.
    \item \textbf{Agent.} A group of $N$ rule-based Bayesian agents each holds a numerical belief.
    \item \textbf{Authority.} An LLM-based Authority, implemented with Llama-3.1-8B-Instruct, collects Agent beliefs via in-context learning, returning individualized responses.
    \item \textbf{Interaction.} Each round, Agents share their beliefs with the Authority, which decide its own belief and communicates it back to each Agent in a numerical format.
    \item \textbf{Update.} Agents update their beliefs by computing a weighted average of their prior belief and the Authority's response, with a trust weight of 0.5. Agents lack direct access to the population belief distribution, relying solely on the Authority's feedback.
\end{itemize}

This setup simulates a realistic scenario where AI mediates collective opinions, potentially amplifying confidence in some beliefs rather than others through feedback loops.

\subsubsection{Setup C: Natural Language Belief Simulation}

This setup uses natural language to represent and communicate value-laden beliefs.

\begin{itemize}
    \item \textbf{Belief} A belief is a natural language statement (e.g., ``Citizens United was the worst thing to happen to the American political landscape.''), sampled from the Changing My View Reddit site.
    \item \textbf{Agent} A group of $N = 10$ simulated users, each implemented using the Llama-3-8B-Instruct model.
    \item \textbf{Authority} An LLM-based Authority, implemented with Llama-3.1-8B-Instruct, processes Agent beliefs via in-context learning and generates its own belief statement.
    \item \textbf{Interaction} Each round, Agents share their belief statements with the Authority, which responds with a natural language belief statement (e.g., ``Citizens United was beneficial, protecting free speech rights.'').
    \item \textbf{Update} Agents consult the Authority and update their beliefs by synthesizing their original stance with the Authority's response.
\end{itemize}

Because beliefs are expressed in natural language, this simulation aims to capture the belief evolution dynamic mediated by LLMs in real life.

